Planning in Strawberry Fields: Evaluating and Improving the Planning and Scheduling Capabilities of LRM o1

The ability to plan a course of action that achieves a desired state of affairs has long been considered a core competence of intelligent agents and has been an integral part of AI research since its inception. With the advent of large language models (LLMs), there has been considerable interest in the question of whether or not they possess such planning abilities, but -- despite the slew of new private and open source LLMs since GPT3 -- progress has remained slow. OpenAI claims that their recent o1 (Strawberry) model has been specifically constructed and trained to escape the normal limitations of autoregressive LLMs -- making it a new kind of model: a Large Reasoning Model (LRM). In this paper, we evaluate the planning capabilities of two LRMs (o1-preview and o1-mini) on both planning and scheduling benchmarks. We see that while o1 does seem to offer significant improvements over autoregressive LLMs, this comes at a steep inference cost, while still failing to provide any guarantees over what it generates. We also show that combining o1 models with external verifiers -- in a so-called LRM-Modulo system -- guarantees the correctness of the combined system's output while further improving performance.

==> figures/o1_obfuscated_randomized.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.5\linewidth]{images/plan_length_vs_correct_zero_shot_obsr.png}
    \caption{Similar to Deceptive Mystery, the performance decreases with plan length significantly, showing problems require more steps might hinder the LRMs.}
    \label{fig:obsr_o1}
\end{figure}

==> figures/o1_reasoning_tokens.tex <==
\begin{figure}[h]
\centering
\includegraphics[width=\linewidth]{images/plan_length_vs_reasoning_tokens_bw.png}
\caption{ \todo{put this and Fig 3 side by side to save space}}
\label{fig:reasoning_tokens}
\end{figure}

==> figures/optimal.tex <==
\begin{figure}
\centering
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{images/plan_length_vs_correct_optimal_o1_preview.png}
  \label{fig:optimal_o1mini}
\end{subfigure}%
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{images/plan_length_vs_correct_optimal_o1_mini.png}
  \label{fig:optimal_o1preview}
\end{subfigure}
\caption{On our smaller instance test set, we find that, when o1 models generate correct plans, they also tend to be optimal. However, this also means that when these model generate non-optimal plans, they also tend to fail to be satisficing.}
\label{fig:optimal}
\end{figure}

==> prompts/bw/os_nl.tex <==
\begin{lstlisting}
I am playing with a set of blocks where I need to arrange the blocks into stacks. Here are the actions I can do

Pick up a block
Unstack a block from on top of another block
Put down a block
Stack a block on top of another block

I have the following restrictions on my actions:
I can only pick up or unstack one block at a time.
I can only pick up or unstack a block if my hand is empty.
I can only pick up a block if the block is on the table and the block is clear. A block is clear if the block has no other blocks on top of it and if the block is not picked up.
I can only unstack a block from on top of another block if the block I am unstacking was really on top of the other block.
I can only unstack a block from on top of another block if the block I am unstacking is clear.
Once I pick up or unstack a block, I am holding the block.
I can only put down a block that I am holding.
I can only stack a block on top of another block if I am holding the block being stacked.
I can only stack a block on top of another block if the block onto which I am stacking the block is clear.
Once I put down or stack a block, my hand becomes empty.

[STATEMENT]
As initial conditions I have that, the red block is clear, the blue block is clear, the yellow block is clear, the hand is empty, the blue block is on top of the orange block, the red block is on the table, the orange block is on the table and the yellow block is on the table.
My goal is to have that the orange block is on top of the blue block.

My plan is as follows:

[PLAN]
unstack the blue block from on top of the orange block
put down the blue block
pick up the orange block
stack the orange block on top of the blue block
[PLAN END]

[STATEMENT]
As initial conditions I have that, the red block is clear, the yellow block is clear, the hand is empty, the red block is on top of the blue block, the yellow block is on top of the orange block, the blue block is on the table and the orange block is on the table.
My goal is to have that the orange block is on top of the red block.

My plan is as follows:

[PLAN]\end{lstlisting}

==> prompts/dmbw/os_nl.tex <==
\begin{lstlisting}
I am playing with a set of objects. Here are the actions I can do

   Attack object
   Feast object from another object
   Succumb object
   Overcome object from another object

I have the following restrictions on my actions:
    To perform Attack action, the following facts need to be true: Province object, Planet object, Harmony.
    Once Attack action is performed the following facts will be true: Pain object.
    Once Attack action is performed the following facts will be false: Province object, Planet object, Harmony.
    To perform Succumb action, the following facts need to be true: Pain object.
    Once Succumb action is performed the following facts will be true: Province object, Planet object, Harmony.    
    Once Succumb action is performed the following facts will be false: Pain object.
    To perform Overcome action, the following needs to be true: Province other object, Pain object.
    Once Overcome action is performed the following will be true: Harmony, Province object, Object Craves other object.
    Once Overcome action is performed the following will be false: Province other object, Pain object.
    To perform Feast action, the following needs to be true: Object Craves other object, Province object, Harmony.
    Once Feast action is performed the following will be true: Pain object, Province other object.
    Once Feast action is performed the following will be false:, Object Craves other object, Province object, Harmony.

[STATEMENT]
As initial conditions I have that, object b craves object c, harmony, planet object a, planet object c, planet object d, province object a, province object b and province object d.
My goal is to have that object c craves object b.

My plan is as follows:

[PLAN]
feast object b from object c
succumb object b
attack object c
overcome object c from object b
[PLAN END]

[STATEMENT]
As initial conditions I have that, object a craves object b, object d craves object c, harmony, planet object b, planet object c, province object a and province object d.
My goal is to have that object c craves object a.

My plan is as follows:

[PLAN]

==============RESPONSE OF o1-preview=================
To achieve your goal of having Object C crave Object A, you can follow this plan:

1. **Feast Object D from Object C**

   - **Preconditions**: 
     - Object D craves Object C (given)
     - Province Object D (given)
     - Harmony (given)
   - **Effects**:
     - Adds Pain to Object D
     - Adds Province to Object C
     - Removes Object D craves Object C
     - Removes Province from Object D
     - Removes Harmony
   
2. **Succumb Object D**

   - **Preconditions**: 
     - Pain Object D (from previous step)
   - **Effects**:
     - Adds Province to Object D
     - Adds Planet to Object D
     - Adds Harmony
     - Removes Pain from Object D

3. **Attack Object C**

   - **Preconditions**: 
     - Province Object C (from the first step)
     - Planet Object C (given)
     - Harmony (restored in the previous step)
   - **Effects**:
     - Adds Pain to Object C
     - Removes Province from Object C
     - Removes Planet from Object C
     - Removes Harmony

4. **Overcome Object C from Object A**

   - **Preconditions**: 
     - Province Object A (given)
     - Pain Object C (from previous step)
   - **Effects**:
     - Adds Harmony
     - Adds Province to Object C
     - Adds Object C craves Object A (your goal)
     - Removes Province from Object A
     - Removes Pain from Object C

By following these steps, you manipulate the states of the objects and the world to fulfill the necessary conditions for each action, ultimately achieving your goal.

**Final Plan:**

1. **Feast Object D from Object C**
2. **Succumb Object D**
3. **Attack Object C**
4. **Overcome Object C from Object A**\end{lstlisting}

